AUPE: Collaborative byzantine fault-tolerant peer-sampling

Peer sampling is a crucial primitive in distributed systems, used to manage overlays and disseminate information in large-scale scenarios such as permissionless blockchain systems. Its purpose is to maintain and regularly update a local and partial snapshot, or view, of the complete system's membership. These protocols are often targeted by malicious actors who aim to disrupt higher-level protocols. Typically, an adversary who controls a set of byzantine nodes attempts to manipulate how legitimate nodes perceive the presence of byzantine ones by increasing their representation in the view of honest nodes. While state-of-the-art byzantine-tolerant peer sampling protocols mitigate this bias, their effectiveness decreases significantly as the number of malicious nodes increases. This paper introduces AUPE, the first collaborative Byzantine-tolerant peer sampling protocol that leverages the presence of trusted nodes, such as Intel's SGX capable devices, to collaboratively track the spread of identifiers in the system and locally debias the representation of byzantine nodes. Simulations with 10,000 nodes demonstrate that AUPE outperforms state-of-the-art solutions, achieving nearperfect resilience even when faced with an adversary controlling 26% of the nodes. Overall, by including as few as 10% of trusted nodes, AUPE increases the tolerance of BRAHMS by up to 60% while limiting the impact of the adversary's attack, even when possessing up to 40% of the nodes.

==> sections/background.tex <==

\section{Background}

\am{You can check from here}

In this section we present some knowledge about gossip-based peer sampling and a well-known peer sampling protocol called Brahms.

\textbf{Gossip-based peer sampling}


Gossip is a way of communicating in large-scale distributed systems that allows information to be spread quickly between nodes. Gossip-based protocols have good properties \cite{b9} such as scalability, load balancing on each node, robustness to node failures, low probability for partitions even when nodes join and leave.

The essential building block of these protocols is the sampling of nodes to find new gossip partners. Thus, the goal of the peer sampling service is to construct a %uniformly randomly 
connected graph by periodically exchanging random and uniform samples of nodes. %. Thus, gossip-based peer sampling protocols 
In fact, these protocols consist of periodic peer-to-peer interactions during which a peer sends its partial knowledge of the active nodes in the system (called view) with information about itself and receives the knowledge of other nodes. This way of requesting information follows a \emph{push-pull} model. The received stream of identifiers allows each node to update its view, which are made of \emph{randomly} selected nodes. This last criterion has been proven to  provide a robust connected graph even in the case of a majority of nodes crashing \cite{b9}. Thus, the peer sampling service maintains a dynamic overlay topology in which partitions can be avoided.

%Peer sampling service brings good properties like the 

%During the the execution of the peer sampling protocol, the graph representing the network evolves to acquire some stable properties and reach a state of convergence. In fact, the size of the outdegree and indegree of nodes tend to match the initial predefined view size of the protocol.



\am{Challenges}
The problem is that a group of nodes acting maliciously and controlled by an attacker share false information with their neighbours. 
For example, if they are asked to share their views, they will generate a fake view composed of the members of their malicious group. 
In this way, they can increase their representation in the whole system and this can help them to gain an advantage for upper layer protocols and even isolate some nodes from the system.

\textbf{Brahms protocol}
%Brahms is a Byzantine fault tolerant protocol which reduce Byzantine pollution with the help of samplers composed of random independent hash functions.

\am{intro}
Brahms \cite{b4} is a gossip-based peer sampling protocol tolerant to Byzantine misbehavior and sybil attacks. The main goal of Brahms is to prevent local views of correct nodes from being exclusively poisoned with Byzantine identifiers. Brahms uses a push-pull gossip-based membership for information dissemination and adds some additional components to enhance its defense mechanism.

\am{Description of Brahms}
Brahms provides to each node in the system with a local view of size $l$, which is a list of identifiers (IDs) and addresses of other nodes. Periodically, each node $i$ selects a fraction $\alpha$ of the identifiers in its view to send PUSH messages containing its own ID to those identifiers. In addition, the node selects a fraction $\beta$ of the identifiers in its view to send PULL messages requesting their views. Each node also has a sampling component, which is a set of $s$ min-wise permutation hash functions randomly chosen by the node at initialization. This component is periodically filled by the received pulled and pushed identifiers to generate a random sample of these nodes. The resulting sample is a sample list $S$, which is a set of $s$ received identifiers that minimize the $s$ hash functions. At the end of the round, the node updates its view by randomly selecting (1) $\alpha \times l$ IDs from the received pushed IDs, (2) $\beta \times l$ IDs from the received pulled IDs and (3) $\gamma \times l$ IDs from the sample list, such that $\alpha + \beta + \gamma = 1$. %random identifiers inside the set of received ones. 
In this work, we set the parameters as recommended in \cite{b4}, with $\alpha=\beta=0.4$ and $\gamma=0.2$.

\am{Do I need to present the other measures of Brahms? As we implemented a light version of it . I think NO}
%Brahms consists of two building blocks:
%\begin{itemize}
 %   \item A gossip component based on a push-pull mechanism. Each node maintains a dynamic view $V$ composed of locally known gossip partners and spreads some of these nodes around the system when responding to PULL messages it received. It can also send information about itself to its neighbours. 
  %  \item Local sampling component. Each node maintains a sample list $S$ of nodes obtained uniformly using min wise independent hash functions.
%\end{itemize}

\am{Results of Brahms and motivation for the article}
With Brahms, partition between correct nodes is avoided under the presence of less than $30\%$ of Byzantine nodes. 
